Search for dark matter and other new phenomena in events with an energetic jet and large missing transverse momentum using the ATLAS detector

Results of a search for new phenomena in final states with an energetic jet and large missing transverse momentum are reported. The search uses proton--proton collision data corresponding to an integrated luminosity of 36.1 fb${}^{-1}$ at a centre-of-mass energy of 13 TeV collected in 2015 and 2016 with the ATLAS detector at the Large Hadron Collider. Events are required to have at least one jet with a transverse momentum above 250 GeV and no leptons ($e$ or $\mu$). Several signal regions are considered with increasing requirements on the missing transverse momentum above 250 GeV. Good agreement is observed between the number of events in data and Standard Model predictions. The results are translated into exclusion limits in models with pair-produced weakly interacting dark-matter candidates, large extra spatial dimensions, and supersymmetric particles in several compressed scenarios.

==> Makefile <==
# Makefile for creating an ATLAS LaTeX document
#------------------------------------------------------------------------------
# By default makes mydocument.pdf using target run_pdflatex.
# Replace mydocument with your main filename or add another target set.
# Adjust TEXLIVE if it is not correct, or pass it to "make new".
# Replace BIBTEX = biber with BIBTEX = bibtex if you use bibtex instead of biber.
# Adjust FIGSDIR for your figures directory tree.
# Adjust the %.pdf dependencies according to your directory structure.
# Use "make clean" to cleanup.
# Use "make cleanpdf" to delete $(BASENAME).pdf.
# "make cleanall" also deletes the PDF file $(BASENAME).pdf.
# Use "make cleanepstopdf" to rmeove PDF files created automatically from EPS files.
#   Note that FIGSDIR has to be set properly for this to work.

# Set the default target to run_latexmk instead of run_pdflatex to use latexmk to compile.

# If you have to run latex rather than pdflatex adjust the dependencies of %.dvi target
#   and use the command "make run_latex" to compile.
# Specify dvipdf or dvips as the run_latex dependency,
#   depending on which you want to use.

#-------------------------------------------------------------------------------
# Check which TeX Live installation you have with the command pdflatex --version
TEXLIVE  = 2016
LATEX    = latex
PDFLATEX = pdflatex
# BIBTEX   = bibtex
BIBTEX   = biber
DVIPS    = dvips
DVIPDF   = dvipdf

#-------------------------------------------------------------------------------
# The main document filename
BASENAME = mono_paper_2017

#-------------------------------------------------------------------------------
# Adjust this according to your top-level figures directory
# This directory tree is used by the "make cleanepstopdf" command
FIGSDIR  = figs
#-------------------------------------------------------------------------------

# EPSTOPDFFILES = `find . -name \*eps-converted-to.pdf`
rwildcard=$(foreach d,$(wildcard $1*),$(call rwildcard,$d/,$2) $(filter $(subst *,%,$2),$d))
EPSTOPDFFILES = $(call rwildcard, $(FIGSDIR), *eps-converted-to.pdf)

# Default target - make mydocument.pdf with pdflatex
default: run_pdflatex
# Use latexmk instead to compile
# default: run_latexmk

.PHONY: run_latexmk
.PHONY: newdocument newdocumenttexmf newnotemetadata newpapermetadata newfiles
.PHONY: draftcover preprintcover newdata
.PHONY: clean cleanpdf help

# Standard pdflatex target
run_pdflatex: $(BASENAME).pdf
	@echo "Made $<"

# Remove -pdf option to run latex instead of pdflatex
run_latexmk:
	latexmk -pdf $(BASENAME)

#-------------------------------------------------------------------------------
# Specify the tex and bib file dependencies for running pdflatex
# If your bib files are not in the main directory adjust this target accordingly
#%.pdf:	%.tex *.tex bib/*.bib
%.pdf:	%.tex *.tex *.bib
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<
#-------------------------------------------------------------------------------

# Default is to make a new paper
new: newnote

newpaper: TEMPLATE=atlas-paper
newpaper: newdocument newfiles newpapermetadata newauxmat

newpapertexmf: TEMPLATE=atlas-paper
newpapertexmf: newdocumenttexmf newfiles newpapermetadata newauxmat

newnote: TEMPLATE=atlas-note
newnote: newdocument newfiles newnotemetadata

newnotetexmf: TEMPLATE=atlas-note
newnotetexmf: newdocumenttexmf newfiles newnotemetadata

newbook: TEMPLATE=atlas-book
newbook: newdocument newfiles newpapermetadata

newbooktexmf: TEMPLATE=atlas-book
newbooktexmf: newdocumenttexmf newfiles newpapermetadata

draftcover:
	if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	  sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' template/atlas-draft-cover.tex \
	    >$(BASENAME)-draft-cover.tex; \
	else \
	  echo "Invalid value for TEXLIVE: $(TEXLIVE)"; \
	  cp  template/$(BASENAME)-draft-cover.tex $(BASENAME)-draft-cover.tex; \
	fi

preprintcover:
	sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' template/atlas-preprint-cover.tex \
	  >$(BASENAME)-preprint-cover.tex
	#cp template/atlas-preprint-cover.tex $(BASENAME)-preprint-cover.tex

newdata:
	sed s/atlas-document/$(BASENAME)/ template/atlas-hepdata-main.tex | \
	sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' >$(BASENAME)-hepdata-main.tex
	cp template/atlas-hepdata.tex $(BASENAME)-hepdata.tex

newdocument:
	if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	  sed s/atlas-document/$(BASENAME)/ template/$(TEMPLATE).tex | \
	    sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' >$(BASENAME).tex; \
	else \
	  echo "Invalid value for TEXLIVE: $(TEXLIVE)"; \
	  sed s/atlas-document/$(BASENAME)/ template/$(TEMPLATE).tex >$(BASENAME).tex; \
	fi

newdocumenttexmf:
	if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	  sed s/atlas-document/$(BASENAME)/ template/$(TEMPLATE).tex | \
	  sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' | \
	  sed 's/\\newcommand\*{\\ATLASLATEXPATH}{latex\/}/% \\newcommand\*{\\ATLASLATEXPATH}{latex\/}/' | \
	  sed 's/% \\newcommand\*{\\ATLASLATEXPATH}{}/\\newcommand\*{\\ATLASLATEXPATH}{}/' \
	  >$(BASENAME).tex; \
	else \
	  echo "Invalid value for TEXLIVE: $(TEXLIVE)"; \
	  sed s/atlas-document/$(BASENAME)/ template/$(TEMPLATE).tex >$(BASENAME).tex; \
	fi

newpapermetadata:
	cp template/atlas-paper-metadata.tex $(BASENAME)-metadata.tex

newnotemetadata:
	cp template/atlas-note-metadata.tex $(BASENAME)-metadata.tex

newfiles:
	echo "% Put you own bibliography entries in this file" > $(BASENAME).bib
	# touch $(BASENAME).bib
	touch $(BASENAME)-defs.sty

newauxmat:
	cp template/atlas-auxmat.tex $(BASENAME)-auxmat.tex
	cp template/atlas-hepdata.tex $(BASENAME)-hepdata.tex

run_latex: dvipdf

# Targets if you run latex instead of pdflatex
dvipdf:	$(BASENAME).dvi
	$(DVIPDF) -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress $<
	@echo "Made $(basename $<).pdf"

dvips:	$(BASENAME).dvi
	$(DVIPS) $<
	@echo "Made $(basename $<).ps"

# Specify dependencies for running latex
#%.dvi:	%.tex tex/*.tex bibtex/bib/*.bib
%.dvi:	%.tex *.tex *.bib
	$(LATEX)    $<
	-$(BIBTEX)  $(basename $<)
	$(LATEX)    $<
	$(LATEX)    $<

%.bbl:	%.tex *.bib
	$(LATEX) $<
	$(BIBTEX) $<

help:
	@echo "To create a new paper/CONF Note/PUB Note draft give the command:"
	@echo "make newpaper [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "To create a new ATLAS note draft give the command:"
	@echo "make newnote [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "To create a long document (book) like a TDR:"
	@echo "make newbook [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo ""
	@echo "To compile the paper give the command"
	@echo "make"
	@echo "If your bib files are not in the main directory, adjust the %.pdf target accordingly." 
	@echo ""
	@echo "To compile the document using latexmk give the command:"
	@echo "make latexmk"
	@echo "You can also adjust the 'default' target."
	@echo ""
	@echo "If atlaslatex is installed centrally, e.g. in ~/texmf:"
	@echo "make newpapertexmf|newnotetexmf|newbooktemf [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo ""
	@echo "If you need a standalone draft cover give the commands:"
	@echo "make draftcover [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "pdflatex mydocument-draft-cover"
	@echo ""
	@echo "If you need a standalone preprint cover give the commands:"
	@echo "make preprintcover [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "pdflatex mydocument-preprint-cover"
	@echo ""
	@echo "If you need a document for HepData material give the commands:"
	@echo "make newdata [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "pdflatex mydocument-hepdata-main"
	@echo ""
	@echo "make clean    to clean auxiliary files (not output PDF)"
	@echo "make cleanpdf to clean output PDF files"
	@echo "make cleanps  to clean output PS files"
	@echo "make cleanall to clean all files"
	@echo "make cleanepstopdf to clean PDF files automatically made from EPS"
	@echo ""

clean:
	-rm *.dvi *.toc *.aux *.log *.out \
		*.bbl *.blg *.brf *.bcf *-blx.bib *.run.xml \
		*.cb *.ind *.idx *.ilg *.inx \
		*.synctex.gz *~ *.fls *.fdb_latexmk .*.lb spellTmp 

cleanpdf:
	-rm $(BASENAME).pdf 
	-rm $(BASENAME)-draft-cover.pdf $(BASENAME)-preprint-cover.pdf
	-rm $(BASENAME)-hepdata-main.pdf

cleanps:
	-rm $(BASENAME).ps 
	-rm $(BASENAME)-draft-cover.ps $(BASENAME)-preprint-cover.ps
	-rm $(BASENAME)-hepdata-main.ps

cleanall: clean cleanpdf cleanps

# Clean the PDF files created automatically from EPS files
cleanepstopdf: $(EPSTOPDFFILES)
	@echo "Removing PDF files made automatically from EPS files"
	-rm $^

